Multiwavelength Observations of the Apparently Non-repeating FRB 20250316A

The physical origin of fast radio bursts (FRBs) remains uncertain. Although multiwavelength observations have been widely conducted, only Galactic FRB~20200428D is associated with an X-ray burst from the magnetar SGR J1935+2154. Here, we present multiwavelength follow-up observations of the nearby bright FRB~20250316A, including the Five-hundred-meter Aperture Spherical radio Telescope (FAST), Einstein Probe (EP) X-ray mission, Chandra X-ray Observatory, Wide Field Survey Telescope (WFST) and Space Variable Object Monitor/Visible Telescope (SVOM/VT). The 13.08-hour FAST follow-up campaign without pulse detection requires an energy distribution flatter than those of well-known repeating FRBs, suggesting that this burst is likely a one-off event. A prompt EP follow-up and multi-epoch observational campaign totaling $>$ 100 ks led to the detection of an X-ray source within the angular resolution of its Follow-up X-ray Telescope (FXT, $10^{\prime\prime}$). A subsequent Chandra observation revealed this source to be offset by $7^{\prime\prime}$ from the FRB position, and established a 0.5-10 keV flux upper limit of $7.6\times 10^{-15}$ $\rm erg\,cm^{-2}\,s^{-1}$ at the FRB position, corresponding to $\sim 10^{39}$ $\rm erg\,s^{-1}$ at the 40 Mpc distance of the host galaxy NGC~4141. These results set one of the most stringent limits on X-ray emission from a non-repeating FRB, disfavoring ultra-luminous X-ray sources (ULXs) as counterparts of apparently one-off FRBs and offering critical insights into afterglow models. Our study suggests that an arcsecond localization of both the FRB and its potential X-ray counterpart is essential for exploring the X-ray counterpart of an FRB.

==> tbopt1img.tex <==
\begin{center}
\scriptsize
\setlength{\tabcolsep}{2 pt}
\begin{longtable}{cccccc}
\caption{Optical Observations and Upper Limits}
\label{tb:opt1img}\\
\hline
No & telescope & start time & MJD & filter & mag$_\mathrm{lim}$ \\
\hline
\endfirsthead
\multicolumn{6}{c}{{\tablename\ \thetable{} -- Continued}} \\
\hline
No & telescope & start time & MJD & filter & mag$_\mathrm{lim}$ \\
\hline
\endhead
\hline
\multicolumn{6}{r}{{Continued on next page}} \\
\endfoot
\hline
\endlastfoot
%No & telescope & start time & MJD & filter & mag$_\mathrm{lim}$ \\
1 & WFST & 2025-03-22T17:04:19.000 & 60756.71133 & $r$ & 23.12 \\
2 & WFST & 2025-03-22T17:07:35.000 & 60756.71360 & $r$ & 23.03 \\
3 & WFST & 2025-03-22T17:10:52.000 & 60756.71588 & $r$ & 23.06 \\
4 & WFST & 2025-03-22T17:14:09.000 & 60756.71816 & $r$ & 23.27 \\
5 & WFST & 2025-03-22T18:00:18.000 & 60756.75021 & $r$ & 23.07 \\
6 & WFST & 2025-03-22T18:03:34.000 & 60756.75248 & $r$ & 23.07 \\
7 & WFST & 2025-03-22T18:06:50.000 & 60756.75475 & $r$ & 23.11 \\
8 & WFST & 2025-03-22T18:10:07.000 & 60756.75703 & $r$ & 22.97 \\
9 & WFST & 2025-03-22T18:13:23.000 & 60756.75929 & $r$ & 22.98 \\
10 & WFST & 2025-03-22T18:19:34.000 & 60756.76359 & $r$ & 22.94 \\
11 & WFST & 2025-03-22T18:22:50.000 & 60756.76586 & $r$ & 23.06 \\
12 & WFST & 2025-03-22T18:26:06.000 & 60756.76813 & $r$ & 23.03 \\
13 & WFST & 2025-03-22T18:29:23.000 & 60756.77041 & $r$ & 23.09 \\
14 & WFST & 2025-03-22T18:32:39.000 & 60756.77267 & $r$ & 23.13 \\
15 & WFST & 2025-03-22T18:35:55.000 & 60756.77494 & $r$ & 23.19 \\
16 & WFST & 2025-03-22T18:39:12.000 & 60756.77722 & $r$ & 23.25 \\
17 & WFST & 2025-03-22T18:42:28.000 & 60756.77949 & $r$ & 23.18 \\
18 & WFST & 2025-03-22T18:45:44.000 & 60756.78176 & $r$ & 23.20 \\
19 & WFST & 2025-03-22T18:49:01.000 & 60756.78404 & $r$ & 23.33 \\
20 & WFST & 2025-03-22T18:55:12.000 & 60756.78833 & $r$ & 23.25 \\
21 & WFST & 2025-03-22T18:58:29.000 & 60756.79061 & $r$ & 23.34 \\
\hline
1 & SVOM/VT & 2025-03-23 18:29:00 & 60757.77014 & VT\_B & 22.03 \\
2 & SVOM/VT & 2025-03-23 18:30:00 & 60757.77083 & VT\_B & 22.03 \\
3 & SVOM/VT & 2025-03-23 18:31:00 & 60757.77153 & VT\_B & 22.03 \\
4 & SVOM/VT & 2025-03-23 18:32:00 & 60757.77222 & VT\_B & 21.98 \\
5 & SVOM/VT & 2025-03-23 18:33:00 & 60757.77292 & VT\_B & 22.00 \\
6 & SVOM/VT & 2025-03-23 18:34:00 & 60757.77361 & VT\_B & 21.99 \\
7 & SVOM/VT & 2025-03-23 18:35:00 & 60757.77431 & VT\_B & 22.06 \\
8 & SVOM/VT & 2025-03-23 18:36:00 & 60757.77500 & VT\_B & 22.00 \\
9 & SVOM/VT & 2025-03-23 18:37:00 & 60757.77569 & VT\_B & 22.04 \\
10 & SVOM/VT & 2025-03-23 18:38:00 & 60757.77639 & VT\_B & 22.00 \\
11 & SVOM/VT & 2025-03-23 18:39:00 & 60757.77708 & VT\_B & 22.06 \\
12 & SVOM/VT & 2025-03-23 18:40:00 & 60757.77778 & VT\_B & 21.94 \\
13 & SVOM/VT & 2025-03-23 18:41:00 & 60757.77847 & VT\_B & 21.99 \\
14 & SVOM/VT & 2025-03-23 18:42:00 & 60757.77917 & VT\_B & 22.01 \\
15 & SVOM/VT & 2025-03-23 18:43:00 & 60757.77986 & VT\_B & 22.01 \\
16 & SVOM/VT & 2025-03-23 18:44:00 & 60757.78056 & VT\_B & 22.08 \\
17 & SVOM/VT & 2025-03-23 18:45:00 & 60757.78125 & VT\_B & 22.01 \\
18 & SVOM/VT & 2025-03-23 18:46:00 & 60757.78194 & VT\_B & 22.02 \\
19 & SVOM/VT & 2025-03-23 18:47:00 & 60757.78264 & VT\_B & 22.02 \\
20 & SVOM/VT & 2025-03-23 18:48:00 & 60757.78333 & VT\_B & 21.91 \\
21 & SVOM/VT & 2025-03-23 18:49:00 & 60757.78403 & VT\_B & 21.90 \\
22 & SVOM/VT & 2025-03-23 18:50:00 & 60757.78472 & VT\_B & 21.99 \\
23 & SVOM/VT & 2025-03-23 18:51:00 & 60757.78542 & VT\_B & 22.01 \\
24 & SVOM/VT & 2025-03-23 18:52:00 & 60757.78611 & VT\_B & 22.01 \\
25 & SVOM/VT & 2025-03-23 18:53:00 & 60757.78681 & VT\_B & 21.98 \\
26 & SVOM/VT & 2025-03-23 18:54:00 & 60757.78750 & VT\_B & 22.00 \\
27 & SVOM/VT & 2025-03-23 18:55:00 & 60757.78819 & VT\_B & 21.95 \\
28 & SVOM/VT & 2025-03-23 18:56:00 & 60757.78889 & VT\_B & 22.03 \\
29 & SVOM/VT & 2025-03-23 18:57:00 & 60757.78958 & VT\_B & 21.99 \\
30 & SVOM/VT & 2025-03-23 18:58:00 & 60757.79028 & VT\_B & 21.99 \\
31 & SVOM/VT & 2025-03-23 18:59:00 & 60757.79097 & VT\_B & 22.04 \\
32 & SVOM/VT & 2025-03-23 19:00:00 & 60757.79167 & VT\_B & 21.98 \\
33 & SVOM/VT & 2025-03-23 19:01:00 & 60757.79236 & VT\_B & 22.05 \\
34 & SVOM/VT & 2025-03-23 20:05:48 & 60757.83736 & VT\_B & 21.93 \\
35 & SVOM/VT & 2025-03-23 20:06:48 & 60757.83806 & VT\_B & 22.02 \\
36 & SVOM/VT & 2025-03-23 20:07:48 & 60757.83875 & VT\_B & 22.08 \\
37 & SVOM/VT & 2025-03-23 20:08:48 & 60757.83944 & VT\_B & 22.01 \\
38 & SVOM/VT & 2025-03-23 20:09:48 & 60757.84014 & VT\_B & 22.04 \\
39 & SVOM/VT & 2025-03-23 20:10:48 & 60757.84083 & VT\_B & 21.95 \\
40 & SVOM/VT & 2025-03-23 20:11:48 & 60757.84153 & VT\_B & 22.05 \\
41 & SVOM/VT & 2025-03-23 20:12:48 & 60757.84222 & VT\_B & 22.03 \\
42 & SVOM/VT & 2025-03-23 20:13:48 & 60757.84292 & VT\_B & 21.92 \\
43 & SVOM/VT & 2025-03-23 20:14:48 & 60757.84361 & VT\_B & 21.99 \\
44 & SVOM/VT & 2025-03-23 20:15:48 & 60757.84431 & VT\_B & 22.09 \\
45 & SVOM/VT & 2025-03-23 20:16:48 & 60757.84500 & VT\_B & 22.03 \\
46 & SVOM/VT & 2025-03-23 20:17:48 & 60757.84569 & VT\_B & 22.08 \\
47 & SVOM/VT & 2025-03-23 20:18:48 & 60757.84639 & VT\_B & 21.94 \\
48 & SVOM/VT & 2025-03-23 20:19:48 & 60757.84708 & VT\_B & 21.98 \\
49 & SVOM/VT & 2025-03-23 20:20:48 & 60757.84778 & VT\_B & 22.02 \\
50 & SVOM/VT & 2025-03-23 20:21:48 & 60757.84847 & VT\_B & 22.01 \\
51 & SVOM/VT & 2025-03-23 20:22:48 & 60757.84917 & VT\_B & 21.96 \\
52 & SVOM/VT & 2025-03-23 20:23:48 & 60757.84986 & VT\_B & 21.95 \\
53 & SVOM/VT & 2025-03-23 20:24:48 & 60757.85056 & VT\_B & 22.04 \\
54 & SVOM/VT & 2025-03-23 20:25:48 & 60757.85125 & VT\_B & 22.04 \\
55 & SVOM/VT & 2025-03-23 20:26:48 & 60757.85194 & VT\_B & 22.01 \\
56 & SVOM/VT & 2025-03-23 20:27:48 & 60757.85264 & VT\_B & 22.01 \\
57 & SVOM/VT & 2025-03-23 20:28:48 & 60757.85333 & VT\_B & 21.95 \\
58 & SVOM/VT & 2025-03-23 20:29:48 & 60757.85403 & VT\_B & 22.10 \\
59 & SVOM/VT & 2025-03-23 20:30:48 & 60757.85472 & VT\_B & 21.96 \\
60 & SVOM/VT & 2025-03-23 20:31:48 & 60757.85542 & VT\_B & 22.01 \\
61 & SVOM/VT & 2025-03-23 20:32:48 & 60757.85611 & VT\_B & 22.03 \\
62 & SVOM/VT & 2025-03-23 20:33:48 & 60757.85681 & VT\_B & 21.94 \\
63 & SVOM/VT & 2025-03-23 20:34:48 & 60757.85750 & VT\_B & 21.99 \\
64 & SVOM/VT & 2025-03-23 20:35:48 & 60757.85819 & VT\_B & 22.00 \\
65 & SVOM/VT & 2025-03-23 20:36:48 & 60757.85889 & VT\_B & 22.05 \\
66 & SVOM/VT & 2025-03-23 20:37:48 & 60757.85958 & VT\_B & 22.02 \\
67 & SVOM/VT & 2025-03-23 20:38:48 & 60757.86028 & VT\_B & 22.00 \\
68 & SVOM/VT & 2025-03-23 21:42:31 & 60757.90453 & VT\_B & 21.98 \\
69 & SVOM/VT & 2025-03-23 21:43:31 & 60757.90522 & VT\_B & 21.99 \\
70 & SVOM/VT & 2025-03-23 21:44:31 & 60757.90591 & VT\_B & 21.91 \\
71 & SVOM/VT & 2025-03-23 21:45:31 & 60757.90661 & VT\_B & 22.05 \\
72 & SVOM/VT & 2025-03-23 21:46:31 & 60757.90730 & VT\_B & 21.97 \\
73 & SVOM/VT & 2025-03-23 21:47:31 & 60757.90800 & VT\_B & 21.92 \\
74 & SVOM/VT & 2025-03-23 21:48:31 & 60757.90869 & VT\_B & 21.98 \\
75 & SVOM/VT & 2025-03-23 21:49:31 & 60757.90939 & VT\_B & 22.06 \\
76 & SVOM/VT & 2025-03-23 21:50:31 & 60757.91008 & VT\_B & 22.01 \\
77 & SVOM/VT & 2025-03-23 21:51:31 & 60757.91078 & VT\_B & 22.00 \\
78 & SVOM/VT & 2025-03-23 21:52:31 & 60757.91147 & VT\_B & 22.02 \\
79 & SVOM/VT & 2025-03-23 21:53:31 & 60757.91216 & VT\_B & 22.03 \\
80 & SVOM/VT & 2025-03-23 21:54:31 & 60757.91286 & VT\_B & 22.00 \\
81 & SVOM/VT & 2025-03-23 21:55:31 & 60757.91355 & VT\_B & 22.07 \\
82 & SVOM/VT & 2025-03-23 21:56:31 & 60757.91425 & VT\_B & 22.05 \\
83 & SVOM/VT & 2025-03-23 21:57:31 & 60757.91494 & VT\_B & 22.06 \\
84 & SVOM/VT & 2025-03-23 21:58:31 & 60757.91564 & VT\_B & 22.05 \\
85 & SVOM/VT & 2025-03-23 21:59:31 & 60757.91633 & VT\_B & 22.03 \\
86 & SVOM/VT & 2025-03-23 22:00:31 & 60757.91703 & VT\_B & 21.98 \\
87 & SVOM/VT & 2025-03-23 22:01:31 & 60757.91772 & VT\_B & 21.98 \\
88 & SVOM/VT & 2025-03-23 22:02:31 & 60757.91841 & VT\_B & 22.05 \\
89 & SVOM/VT & 2025-03-23 22:03:31 & 60757.91911 & VT\_B & 22.04 \\
90 & SVOM/VT & 2025-03-23 22:04:31 & 60757.91980 & VT\_B & 22.05 \\
91 & SVOM/VT & 2025-03-23 22:05:31 & 60757.92050 & VT\_B & 21.99 \\
92 & SVOM/VT & 2025-03-23 22:06:31 & 60757.92119 & VT\_B & 21.99 \\
93 & SVOM/VT & 2025-03-23 22:07:31 & 60757.92189 & VT\_B & 21.98 \\
94 & SVOM/VT & 2025-03-23 22:08:31 & 60757.92258 & VT\_B & 22.07 \\
95 & SVOM/VT & 2025-03-23 22:09:31 & 60757.92328 & VT\_B & 22.00 \\
96 & SVOM/VT & 2025-03-23 22:10:31 & 60757.92397 & VT\_B & 22.01 \\
97 & SVOM/VT & 2025-03-23 22:11:31 & 60757.92466 & VT\_B & 21.97 \\
98 & SVOM/VT & 2025-03-23 22:12:31 & 60757.92536 & VT\_B & 22.01 \\
99 & SVOM/VT & 2025-03-23 22:13:31 & 60757.92605 & VT\_B & 22.00 \\
100 & SVOM/VT & 2025-03-23 22:14:31 & 60757.92675 & VT\_B & 22.03 \\
101 & SVOM/VT & 2025-03-23 22:15:31 & 60757.92744 & VT\_B & 21.99 \\
\hline
1 & SVOM/VT & 2025-03-23 18:29:00 & 60757.77014 & VT\_R & 21.81 \\
2 & SVOM/VT & 2025-03-23 18:30:00 & 60757.77083 & VT\_R & 21.77 \\
3 & SVOM/VT & 2025-03-23 18:31:00 & 60757.77153 & VT\_R & 21.86 \\
4 & SVOM/VT & 2025-03-23 18:32:00 & 60757.77222 & VT\_R & 21.90 \\
5 & SVOM/VT & 2025-03-23 18:33:00 & 60757.77292 & VT\_R & 21.92 \\
6 & SVOM/VT & 2025-03-23 18:34:00 & 60757.77361 & VT\_R & 21.90 \\
7 & SVOM/VT & 2025-03-23 18:35:00 & 60757.77431 & VT\_R & 21.86 \\
8 & SVOM/VT & 2025-03-23 18:36:00 & 60757.77500 & VT\_R & 21.92 \\
9 & SVOM/VT & 2025-03-23 18:37:00 & 60757.77569 & VT\_R & 21.79 \\
10 & SVOM/VT & 2025-03-23 18:38:00 & 60757.77639 & VT\_R & 21.78 \\
11 & SVOM/VT & 2025-03-23 18:39:00 & 60757.77708 & VT\_R & 21.96 \\
12 & SVOM/VT & 2025-03-23 18:40:00 & 60757.77778 & VT\_R & 21.83 \\
13 & SVOM/VT & 2025-03-23 18:41:00 & 60757.77847 & VT\_R & 21.88 \\
14 & SVOM/VT & 2025-03-23 18:42:00 & 60757.77917 & VT\_R & 21.84 \\
15 & SVOM/VT & 2025-03-23 18:43:00 & 60757.77986 & VT\_R & 21.85 \\
16 & SVOM/VT & 2025-03-23 18:44:00 & 60757.78056 & VT\_R & 21.97 \\
17 & SVOM/VT & 2025-03-23 18:45:00 & 60757.78125 & VT\_R & 21.91 \\
18 & SVOM/VT & 2025-03-23 18:46:00 & 60757.78194 & VT\_R & 21.88 \\
19 & SVOM/VT & 2025-03-23 18:47:00 & 60757.78264 & VT\_R & 21.90 \\
20 & SVOM/VT & 2025-03-23 18:48:00 & 60757.78333 & VT\_R & 21.88 \\
21 & SVOM/VT & 2025-03-23 18:49:00 & 60757.78403 & VT\_R & 21.82 \\
22 & SVOM/VT & 2025-03-23 18:50:00 & 60757.78472 & VT\_R & 21.83 \\
23 & SVOM/VT & 2025-03-23 18:51:00 & 60757.78542 & VT\_R & 21.90 \\
24 & SVOM/VT & 2025-03-23 18:52:00 & 60757.78611 & VT\_R & 21.87 \\
25 & SVOM/VT & 2025-03-23 18:53:00 & 60757.78681 & VT\_R & 21.92 \\
26 & SVOM/VT & 2025-03-23 18:54:00 & 60757.78750 & VT\_R & 21.96 \\
27 & SVOM/VT & 2025-03-23 18:55:00 & 60757.78819 & VT\_R & 21.79 \\
28 & SVOM/VT & 2025-03-23 18:56:00 & 60757.78889 & VT\_R & 21.90 \\
29 & SVOM/VT & 2025-03-23 18:57:00 & 60757.78958 & VT\_R & 21.94 \\
30 & SVOM/VT & 2025-03-23 18:58:00 & 60757.79028 & VT\_R & 21.87 \\
31 & SVOM/VT & 2025-03-23 18:59:00 & 60757.79097 & VT\_R & 21.93 \\
32 & SVOM/VT & 2025-03-23 19:00:00 & 60757.79167 & VT\_R & 21.87 \\
33 & SVOM/VT & 2025-03-23 19:01:00 & 60757.79236 & VT\_R & 21.96 \\
34 & SVOM/VT & 2025-03-23 20:05:48 & 60757.83736 & VT\_R & 21.83 \\
35 & SVOM/VT & 2025-03-23 20:06:48 & 60757.83806 & VT\_R & 21.90 \\
36 & SVOM/VT & 2025-03-23 20:07:48 & 60757.83875 & VT\_R & 21.86 \\
37 & SVOM/VT & 2025-03-23 20:08:48 & 60757.83944 & VT\_R & 21.87 \\
38 & SVOM/VT & 2025-03-23 20:09:48 & 60757.84014 & VT\_R & 21.91 \\
39 & SVOM/VT & 2025-03-23 20:10:48 & 60757.84083 & VT\_R & 21.76 \\
40 & SVOM/VT & 2025-03-23 20:11:48 & 60757.84153 & VT\_R & 21.91 \\
41 & SVOM/VT & 2025-03-23 20:12:48 & 60757.84222 & VT\_R & 21.89 \\
42 & SVOM/VT & 2025-03-23 20:13:48 & 60757.84292 & VT\_R & 21.85 \\
43 & SVOM/VT & 2025-03-23 20:14:48 & 60757.84361 & VT\_R & 21.86 \\
44 & SVOM/VT & 2025-03-23 20:15:48 & 60757.84431 & VT\_R & 21.90 \\
45 & SVOM/VT & 2025-03-23 20:16:48 & 60757.84500 & VT\_R & 21.86 \\
46 & SVOM/VT & 2025-03-23 20:17:48 & 60757.84569 & VT\_R & 21.85 \\
47 & SVOM/VT & 2025-03-23 20:18:48 & 60757.84639 & VT\_R & 21.92 \\
48 & SVOM/VT & 2025-03-23 20:19:48 & 60757.84708 & VT\_R & 21.83 \\
49 & SVOM/VT & 2025-03-23 20:20:48 & 60757.84778 & VT\_R & 21.81 \\
50 & SVOM/VT & 2025-03-23 20:21:48 & 60757.84847 & VT\_R & 21.90 \\
51 & SVOM/VT & 2025-03-23 20:22:48 & 60757.84917 & VT\_R & 21.90 \\
52 & SVOM/VT & 2025-03-23 20:23:48 & 60757.84986 & VT\_R & 21.81 \\
53 & SVOM/VT & 2025-03-23 20:24:48 & 60757.85056 & VT\_R & 21.94 \\
54 & SVOM/VT & 2025-03-23 20:25:48 & 60757.85125 & VT\_R & 21.92 \\
55 & SVOM/VT & 2025-03-23 20:26:48 & 60757.85194 & VT\_R & 21.93 \\
56 & SVOM/VT & 2025-03-23 20:27:48 & 60757.85264 & VT\_R & 21.77 \\
57 & SVOM/VT & 2025-03-23 20:28:48 & 60757.85333 & VT\_R & 21.89 \\
58 & SVOM/VT & 2025-03-23 20:29:48 & 60757.85403 & VT\_R & 22.00 \\
59 & SVOM/VT & 2025-03-23 20:30:48 & 60757.85472 & VT\_R & 21.97 \\
60 & SVOM/VT & 2025-03-23 20:31:48 & 60757.85542 & VT\_R & 21.94 \\
61 & SVOM/VT & 2025-03-23 20:32:48 & 60757.85611 & VT\_R & 21.89 \\
62 & SVOM/VT & 2025-03-23 20:33:48 & 60757.85681 & VT\_R & 21.81 \\
63 & SVOM/VT & 2025-03-23 20:34:48 & 60757.85750 & VT\_R & 21.89 \\
64 & SVOM/VT & 2025-03-23 20:35:48 & 60757.85819 & VT\_R & 21.90 \\
65 & SVOM/VT & 2025-03-23 20:36:48 & 60757.85889 & VT\_R & 21.97 \\
66 & SVOM/VT & 2025-03-23 20:37:48 & 60757.85958 & VT\_R & 21.94 \\
67 & SVOM/VT & 2025-03-23 20:38:48 & 60757.86028 & VT\_R & 21.84 \\
68 & SVOM/VT & 2025-03-23 21:42:31 & 60757.90453 & VT\_R & 21.83 \\
69 & SVOM/VT & 2025-03-23 21:43:31 & 60757.90522 & VT\_R & 21.84 \\
70 & SVOM/VT & 2025-03-23 21:44:31 & 60757.90591 & VT\_R & 21.79 \\
71 & SVOM/VT & 2025-03-23 21:45:31 & 60757.90661 & VT\_R & 21.91 \\
72 & SVOM/VT & 2025-03-23 21:46:31 & 60757.90730 & VT\_R & 21.89 \\
73 & SVOM/VT & 2025-03-23 21:47:31 & 60757.90800 & VT\_R & 21.82 \\
74 & SVOM/VT & 2025-03-23 21:48:31 & 60757.90869 & VT\_R & 21.90 \\
75 & SVOM/VT & 2025-03-23 21:49:31 & 60757.90939 & VT\_R & 21.95 \\
76 & SVOM/VT & 2025-03-23 21:50:31 & 60757.91008 & VT\_R & 21.91 \\
77 & SVOM/VT & 2025-03-23 21:51:31 & 60757.91078 & VT\_R & 21.80 \\
78 & SVOM/VT & 2025-03-23 21:52:31 & 60757.91147 & VT\_R & 21.86 \\
79 & SVOM/VT & 2025-03-23 21:53:31 & 60757.91216 & VT\_R & 21.85 \\
80 & SVOM/VT & 2025-03-23 21:54:31 & 60757.91286 & VT\_R & 21.91 \\
81 & SVOM/VT & 2025-03-23 21:55:31 & 60757.91355 & VT\_R & 21.95 \\
82 & SVOM/VT & 2025-03-23 21:56:31 & 60757.91425 & VT\_R & 21.92 \\
83 & SVOM/VT & 2025-03-23 21:57:31 & 60757.91494 & VT\_R & 21.93 \\
84 & SVOM/VT & 2025-03-23 21:58:31 & 60757.91564 & VT\_R & 21.89 \\
85 & SVOM/VT & 2025-03-23 21:59:31 & 60757.91633 & VT\_R & 21.95 \\
86 & SVOM/VT & 2025-03-23 22:00:31 & 60757.91703 & VT\_R & 21.88 \\
87 & SVOM/VT & 2025-03-23 22:01:31 & 60757.91772 & VT\_R & 21.77 \\
88 & SVOM/VT & 2025-03-23 22:02:31 & 60757.91841 & VT\_R & 21.99 \\
89 & SVOM/VT & 2025-03-23 22:03:31 & 60757.91911 & VT\_R & 21.95 \\
90 & SVOM/VT & 2025-03-23 22:04:31 & 60757.91980 & VT\_R & 21.98 \\
91 & SVOM/VT & 2025-03-23 22:05:31 & 60757.92050 & VT\_R & 21.85 \\
92 & SVOM/VT & 2025-03-23 22:06:31 & 60757.92119 & VT\_R & 21.78 \\
93 & SVOM/VT & 2025-03-23 22:07:31 & 60757.92189 & VT\_R & 21.91 \\
94 & SVOM/VT & 2025-03-23 22:08:31 & 60757.92258 & VT\_R & 21.87 \\
95 & SVOM/VT & 2025-03-23 22:09:31 & 60757.92328 & VT\_R & 21.94 \\
96 & SVOM/VT & 2025-03-23 22:10:31 & 60757.92397 & VT\_R & 21.88 \\
97 & SVOM/VT & 2025-03-23 22:11:31 & 60757.92466 & VT\_R & 21.88 \\
98 & SVOM/VT & 2025-03-23 22:12:31 & 60757.92536 & VT\_R & 21.93 \\
99 & SVOM/VT & 2025-03-23 22:13:31 & 60757.92605 & VT\_R & 21.95 \\
100 & SVOM/VT & 2025-03-23 22:14:31 & 60757.92675 & VT\_R & 21.88 \\
101 & SVOM/VT & 2025-03-23 22:15:31 & 60757.92744 & VT\_R & 21.88 \\
\hline
\hline
\end{longtable}
\end{center}

